Torque Responsive Metamaterials Enable High Payload Soft Robot Arms

Soft robots have struggled to support large forces and moments while also supporting their own weight against gravity. This limits their ability to reach certain configurations necessary for tasks such as inspection and pushing objects up. We have overcome this limitation by creating an electrically driven metamaterial soft arm using handed shearing auxetics (HSA) and bendable extendable torque resistant (BETR) shafts. These use the large force and torque capacity of HSAs and the nestable torque transmission of BETRs to create a strong soft arm. We found that the HSA arm was able to push 2.3 kg vertically and lift more than 600 g when positioned horizontally, supporting 0.33 Nm of torque at the base. The arm is able to move between waypoints while carrying the large payload and demonstrates consistent movement with path variance below 5 mm. The HSA arm's ability to perform active grasping with HSA grippers was also demonstrated, requiring 20 N of pull force to dislodge the object. Finally, we test the arm in a pipe inspection task. The arm is able to locate all the defects while sliding against the inner surface of the pipe, demonstrating its compliance.

==> design_methods.tex <==
\section{Design of Metamaterial Soft Robot Arm}

\begin{figure*}
    \centering
    \includegraphics[width=0.99\textwidth]{media/HSA_Arm_HSA_Characterization.png}
    \caption[HSA Characterization]{Interpolated HSA force and torque characterization is presented here for each of the four layers of HSA in the soft arm. Thick-  and thin-walled HSAs printed at 0\% of way along the auxetic trajectory are presented with just expansion data (layer 3, 4 respectively) and HSAs printed beyond that (layer 1, 2) are shown with both expansion and compression regions.}
    \label{fig:HSAARMCharacterization}
    %\vspace{-0.4cm}
\end{figure*}
\begin{table*}[]
\centering
\caption{Table showing the minimum and maximum force (F) and torque ($\tau$) values for all the HSA configurations from the mechanical characterization data. Here, $\theta$ represents the corresponding value of rotation and \textbf{e} represents the corresponding value of extension. The table is divided into two categories to represent the values in the compression and expansion regimes.}
\label{tab:HSACharacterizationTable}
\setlength{\tabcolsep}{20pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{ccccc}
\multicolumn{5}{c}{\textbf{COMPRESSION}}                                                                                  \\ \hline
\textbf{HSA Type} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Min. Force ($\theta$, e)\\ {[}N{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Max. Force ($\theta$, e)\\ {[}N{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Min. Torque ($\theta$, e)\\ {[}Nmm{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Max. Torque ($\theta$, e)\\ {[}Nmm{]}\end{tabular}} \\ \hline
50\%                 & -79.5 (0, -2.6)      & 167.3 (-49.9, 0)     & -120.3 (0, -2.6)     & 275.8 (-49.9, 0)     \\
15\%                 & -34.5 (0, -10.4)     & 38.3 (-29.9, 0)      & -130.2 (-29.9, 0)    & 110.89 (0, -10.4)    \\
0\% (Thick)          & -                    & -                    & -                    & -                    \\
0\% (Thin)           & -                    & -                    & -                    & -                    \\ \hline
\\
\multicolumn{5}{c}{\textbf{EXPANSION}}                                                                                    \\ \hline
\textbf{HSA Type} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Min. Force ($\theta$, e)\\ {[}N{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Max. Force ($\theta$, e)\\ {[}N{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Min. Torque ($\theta$, e)\\ {[}Nmm{]}\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Max. Torque ($\theta$, e)\\ {[}Nmm{]}\end{tabular}} \\ \hline
50\%                 & 0 (0, 0)             & 478.1 (0, 15.7)      & -8.8 (59.9, 0)       & 392.2 (0, 10.4)      \\
15\%                 & -26.3 (29.9, 0)      & 82.5 (0, 20.4)       & -153.29 (0, 10.2)    & 87.9 (9.9, 20.4)     \\
0\% (Thick)          & -27.9 (42, 0)        & 39.7 (0, 13.6)       & -134.8 (0, 13.6)     & 131 (31.3, 0)        \\
0\% (Thin)           & -11.21 (59.9, 0)     & 13.1 (0, 15.3)       & -40.2 (0, 15.3)      & 47 (19.9, 0)         \\ \hline
\end{tabular}
\end{table*}
This section describes the design of our four layer soft metamaterial robot arm. First, we use a lumped element model to determine component performance targets for horizontal payloads of 500 g and 2 kg vertically. Then, we manufacture and test components for both extension performance and torque transmission. We finally evaluate the assembled system to see how well it meets the initial design requirements.

\subsection{HSA Characterization}
%% Component Characterization


Using kinematics, we determined force and torque targets corresponding to a 2 kg vertical lift and a 500 g horizontal lift. Based on work from \cite{good2021expanding,truby2021recipe}, we designed HSAs to achieve the target properties, then manufactured them as described in \ref{characterization}.

We characterize HSAs using two main properties, force (F) and torque ($\tau$) as a function of both displacement and rotation. This extends the characterization from \cite{good2021expanding,truby2021recipe} by characterizing properties beyond the minimum energy state. We characterize four different configurations of the HSA, 50\% open, 15\% open, 0\% open, and 0\% open with thinner walls. These represent the four layers of the arm. The 50\% open HSAs occupied the first layer of the arm, 15\% open HSAs occupied the second layer, and the 0\% HSAs occupied layers three and four as shown in Fig. \ref{fig:SystemLayerOverview}. For layer 4, we reduced the wall thickness of the HSA to reduce the torque requirement for actuation. All of the HSAs on layers 1, 2 and 3 (50\%, 15\%, 0\%) had a length of 90.5 mm, an outer diameter of 30.7 mm, and a wall thickness of 3.5 mm. Layer 4 HSAs (0\%) had the same length and outer diameter with a reduced wall thickness of 1.7 mm.

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{media/HSA_Arm_BETR_Characterization.png}
    \caption[Torque Transmission Characterization]{Plot of torsion and extension tests for the soft soft torque transmission elements in the robot arm. We characterize elements for layer 2 (Small: Short), layer 3 (Large BETR), and layer 4 (Small: Long). We also characterize the single non-extendable flex shaft for complete individual component level analysis. Torque characterization was done when in the extended (dashed) and rest states (solid). The X intercept represents the slack/deadband in the material and the slope represents the torsional stiffness. Forces required to extend the elements in the arm are also shown in the extension test plot. These values oppose HSA extension.
    }
    \label{fig:BETRCharacterization}
    \vspace{-0.2cm}
\end{figure*}

\subsection{Transmission Characterization} \label{characterization}

All HSAs we characterized were fabricated using the Carbon M1 3D printer with FPU 50. All HSAs were printed horizontally on the build platform, and were post processed following the manufacturer's guidelines and specifications.

The test procedure consisted of a series of extensions and rotations that were programmed using a custom test method on an Instron 68SC-2 at 200 Hz. We individually chose the extension and rotation values based on the maximum safe limits of the tested HSA configurations. The ranges of extension and rotation were determined by manually observing them for all HSA configurations. The data was collected over seven and fourteen equidistantly spaced points in displacement and rotation respectively. This results in 98 datapoint groups per HSA. Each datapoint group was collected during a 1 mm vertical displacement at 10 mm/s. The raw data collected from the test apparatus was approximated using cubic fits for displacement and rotation to visualize the force (F) and torque ($\tau$) responses of the HSA as shown in Fig. \ref{fig:HSAARMCharacterization}.

A linear interpolation surface fit was chosen to visualize the data. For the force plot, positive values represent the HSA pulling on the environment while negative values represent pushing on the environment. For torque, positive values represent the HSA trying to twist less in the direction it is twisting and negative values represent the HSA trying to twist more than the direction it is twisting in. The maximum and minimum force and torque values observed for each HSA configuration is shown in Table \ref{tab:HSACharacterizationTable}. 


To deliver torque to layers two through four, a bendable, extendable torque transmission system is needed. We looked to the work presented in \cite{Thomas2025BETR}. We characterized three different configurations of the extendable flex shafts (BETRs), large, long, and short. We characterized their force and torque responses using an Instron 68SC-2 mechanical testing machine. As these BETRs are intended for transmitting torque from the motors to the HSAs, we evaluated the torsional stiffness of these BETRs, while also testing the force required to extend them. Additionally, we incorporated a non-extensible flex shaft at the first layer of the arm to provide enhanced torsional stiffness, while the extendable BETRs were used for the second and third layer. The CAD rendering of the BETR designs can be seen in Fig. \ref{fig:SystemLayerOverview}. The large BETR had an outer diameter of 30.7 mm and a wall thickness of 4.5 mm. They were fabricated with PTFE tubes using a Bantam Desktop CNC machine. The large BETRs were utilized to drive the arm's third layer. Additionally, we fabricated two variants of small BETRs, short and long. The small BETRs were made out of FPU 50 using a Carbon M1 3D printer, and can be seen in Fig. \ref{fig:BETRCharacterization}. The long BETR was fabricated by connecting two short BETRs and a single non-extendable flex shaft using 3D-printed adaptors made out of PLA. The short BETRs were used to drive the 15\% HSAs on the second layer of the HSA arm, while the long BETRs were used to drive the 0\% HSAs on layer 4 as shown in Fig. \ref{fig:SystemLayerOverview}.

The torque response was recorded for the large, short, and long BETRs and the non-extendable flex shaft by applying a rotation of 5 degrees at a rate of 1 deg/s. This characterization was done in both non-extended and extended states for each of the components to understand how torsional stiffness changes with extension. Little change was observed for the BETRs. The large, long, and short BETRs were extended to 45 mm, 35 mm, and 20 mm respectively, while the non-extendable flex shaft was extended to 4 mm. Similarly, for force response, an extension of 22 mm, 20 mm, 35 mm and 5 mm was used for the large, short, long, and non-extensible flex shaft respectively at the rate of 1 mm/s. All of the recorded data were visualized and can be seen in Fig. \ref{fig:BETRCharacterization}.

The torsional stiffness values were then calculated from raw data for each of the BETRs. The large BETR had torsional stiffness values of -11.52 Nmm/deg and -12.03 Nmm/deg at the non-extended and extended states respectively. The long BETR was at -1.39 Nmm/deg and -1.33 Nmm/deg at the non-extended and extended states, showing very little difference in its performance. The short BETR had torsional stiffness values of -3.60 Nmm/deg and -2.90 Nmm/deg at its non-extended and extended states. The non-extendable flex shaft had torsional stiffness values of -3.29 Nmm/deg and -4.78 Nmm/deg at the non-extended and extended states respectively.


\subsection{Fabrication of the Soft Arm} \label{Fabrication of Soft Arm}
In this section, we describe the manufacturing and characterization of the Handed Shearing Auxetic (HSA) actuators, and Bendable Extendable Torsionally-Rigid (BETR) flex shafts. We also describe the fabrication and assembly steps for the HSA arm. We then describe the test methods that were used to evaluate the performance of the robot arm.

A parallel plate system was used to connect the sixteen independent Quasi-Direct Drive motors (QDD100 Beta 3) to the HSAs and BETRs through pulleys. Two torques were transmitted along the same shaft using a set of live and dead axle pulleys with the motors preventing unwanted cross-talk. This forms the metal base at the bottom of the robot that the soft arm is built on top of. 

The components used for the fabrication of the robot arm can be seen in Fig. \ref{fig:SystemLayerOverview}. The HSA arm is made from four levels or layers, where each level was connected to the other layer using 3D-printed plate sections.

For the first level, we added four large BETRs (lavender) with one in each section that drives another four large BETRs at level 2. The large BETRs drive the 0\% HSA (gold) at level 3. Long BETRs (teal) run through the inner sections of the large BETR up to level 4 to drive the thinner HSAs (purple) at the distal end. Levels 1 and 2 are driven using 50\% (yellow) and 15\% (pink) HSAs at levels 1 and 2 respectively. In order to maximize force output, the HSAs were connected to 3D-printed adaptors at levels 1 and 2 as shown in gray in Fig. \ref{fig:SystemLayerOverview}.
